Bilingual Streaming ASR with Grapheme units and Auxiliary Monolingual Loss

We introduce a bilingual solution to support English as secondary locale for most primary locales in hybrid automatic speech recognition (ASR) settings. Our key developments constitute: (a) pronunciation lexicon with grapheme units instead of phone units, (b) a fully bilingual alignment model and subsequently bilingual streaming transformer model, (c) a parallel encoder structure with language identification (LID) loss, (d) parallel encoder with an auxiliary loss for monolingual projections. We conclude that in comparison to LID loss, our proposed auxiliary loss is superior in specializing the parallel encoders to respective monolingual locales, and that contributes to stronger bilingual learning. We evaluate our work on large-scale training and test tasks for bilingual Spanish (ES) and bilingual Italian (IT) applications. Our bilingual models demonstrate strong English code-mixing capability. In particular, the bilingual IT model improves the word error rate (WER) for a code-mix IT task from 46.5% to 13.8%, while also achieving a close parity (9.6%) with the monolingual IT model (9.5%) over IT tests.

==> somebackup.tex <==

% With widespread adoption of ASR in real-life situations, we expect ASR to work across acoustics and speech tasks \cite{hinton2012deep,Deng2013RecentAI, CDDNN_TASLP12}. It's well known that data is oxygen for training deep learning (\textbf{DL}) models, so besides model innovations  \cite{Hochreiter1997long, Sak2014long,sak2015fast, sainath2015convolutional, sak2017recurrent}, 

%Our shared units across locales enable a single multilingual Softmax output state and extend a related work in \cite{huang2013cross}, where the output units were locale-dependent. 
% We scope our work in the domain of TL and develop new TL paradigms with a focus on designing new model units for greater gains for target locales. In sec.~\ref{Sec:Motivation} we motivate a large-scale multilingual pre-train embedding acoustic model (\textbf{AM}) as source  AM to bootstrap target locales with those embeddings. A fully multilingual model can simultaneously support ASR and other speech applications in multiple languages. 

%\cite{Chorowski-AttentionASR}

%Our objective in this work is to develop new acoustic model (AM) architectures to better meet ASR metrics in accuracy, latency and computational cost. We have already noted a progression of model structures in GRU \cite{chung2014empirical}, LSTM \cite{sak2014long_rep}, BLSTM \cite{schuster1997bidirectional, graves2005bidirectional}, LC-BLSTM \cite{chen2016training,xue2017improving}, cLTLSTM \cite{li2019improving}, and F\&S AM \cite{kskumar_FastSlow} with respective trade-offs in aforementioned ASR metrics. BLSTMs provide substantial gains over LSTMs. LC-BLSTMs constrain latency, retain a close accuracy parity with BLSTM models,  thus provide an approach to high accuracy streaming ASR solution.

